Two-stage LLM Fine-tuning with Less Specialization and More Generalization

Pretrained large language models (LLMs) are general purpose problem solvers applicable to a diverse set of tasks with prompts. They can be further improved towards a specific task by fine-tuning on a specialized dataset. However, fine-tuning usually makes the model narrowly specialized on this dataset with reduced general in-context learning performances, which is undesirable whenever the fine-tuned model needs to handle additional tasks where no fine-tuning data is available. In this work, we first demonstrate that fine-tuning on a single task indeed decreases LLMs' general in-context learning performance. We discover one important cause of such forgetting, format specialization, where the model overfits to the format of the fine-tuned task.We further show that format specialization happens at the very beginning of fine-tuning. To solve this problem, we propose Prompt Tuning with MOdel Tuning (ProMoT), a simple yet effective two-stage fine-tuning framework that reduces format specialization and improves generalization.ProMoT offloads task-specific format learning into additional and removable parameters by first doing prompt tuning and then fine-tuning the model itself with this soft prompt attached. With experiments on several fine-tuning tasks and 8 in-context evaluation tasks, we show that ProMoT achieves comparable performance on fine-tuned tasks to standard fine-tuning, but with much less loss of in-context learning performances across a board range of out-of-domain evaluation tasks. More importantly, ProMoT can even enhance generalization on in-context learning tasks that are semantically related to the fine-tuned task, e.g. ProMoT on En-Fr translation significantly improves performance on other language pairs, and ProMoT on NLI improves performance on summarization. Experiments also show that ProMoT can improve the generalization performance of multi-task training.

==> apd_enfr.tex <==
\begin{table}[!htbp]
    \centering
    \caption{Results of model trained on WMT14 En-Fr dataset. For RTE, CB and WiC, we report the results from development set. For other datasets, we report the results on test set. We list the accuracy on fine-tuning target task (En-Fr) on the first row. Here 1-shot Two-stage denotes running our two-stage fine-tune strategy on En-Fr dataset with 1-shot prompt.}
    \adjustbox{max width=\textwidth}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c}
    \toprule
         Datasets & \multicolumn{2}{c|}{Prompt-tuning} & \multicolumn{2}{c|}{Model Fine-tuning} & \multicolumn{2}{c|}{Two-stage (Ours)} & \multicolumn{2}{c}{1-shot Two-stage (Ours)}\\
    \midrule
         WMT14 En-Fr & \multicolumn{2}{c|}{39.28} & \multicolumn{2}{c|}{43.62} & \multicolumn{2}{c|}{41.3} & \multicolumn{2}{c}{41.19}\\
    \midrule
         & 1-shot & 4-shots & 1-shot & 4-shots & 1-shot & 4-shots & 1-shot & 4-shots\\
    \midrule
         CB& 46.43 & 51.79 & 25.6 & 23.214 & 41.071 & 57.143 & 41.071&53.571\\
         WiC & 49.687 & 49.687 & 18.714 & 46.395 & 50.157 & 50.313&49.843&50.627\\
         triviaQA  & 17.582 & 19.022 & 0.027 & 0.00 & 13.63 & 15.204&16.927&18.191\\
         web\_questions & 9.695 & 13.041 & 0.049& 0.00 & 9.4 & 7.923&10.138&12.008\\
         WMT16\_ende & 3.974 & 8.83 & 0.668 & 0.126 & 15.517 & 15.548&16.139&15.626\\
         WMT16\_enro & 1.818 & 3.918 & 0.912 & 0.137 & 18.544 & 17.799&17.568&16.808\\
         XSum & 6.410 & 2.353 & 0.181 & 0.063 & 1.493 & 0.65&3.407&4.362\\
         WikiLingua & 4.585 & 1.329 & 0.034 & 0.005 & 1.142 & 0.524&4.215&4.727\\
    \bottomrule
    \end{tabular}
    }
    \label{tab:apd_single_enfr}
\end{table}

==> app_table_flan_t5_RTE.tex <==
\begin{table*}[!htbp]
    \centering
    \caption{In-context performance of FLAN-T5 XXL finetuned on RTE and evaluated on 8 few-shot tasks. The accuracy on fine-tuned task (RTE) is in the first row. Prompt-tuning doesn't modify pretrained model parameters and has the same in-context performance as pretrained model. 
    % \daliangli{are we still going to seperate pretraining with prompt-tuning?}
    }
    
    \adjustbox{max width=\textwidth}{
    \begin{tabular}{c|c|c|c|c}
    \toprule
         Datasets & \multicolumn{1}{c|}{Pretrained} &\multicolumn{1}{c|}{Prompt-tuning} & \multicolumn{1}{c|}{Standard Fine-tuning} & \multicolumn{1}{c}{ProMoT (Ours)}\\
    \midrule
         RTE & \multicolumn{1}{c|}{-} &\multicolumn{1}{c|}{93.86} & \multicolumn{1}{c|}{94.22} & \multicolumn{1}{c}{94.22}\\
    % \midrule
    %      & 1-shot & 4-shots& 1-shot & 4-shots & 1-shot & 4-shots & 1-shot & 4-shots & 1-shot & 4-shots\\
    \midrule
         CB& 83.929&83.929&85.714&	83.929\\
         WiC & 61.755&61.755&67.085&62.069\\
         triviaQA  & 33.926&33.926&36.241&33.926\\
         web\_questions & 34.744&34.744&33.612&34.695\\
         WMT16\_ende & 11.591&11.591&9.987&11.719\\
         WMT16\_enro & 16.806&16.806&14.816&16.725\\
         XSum & 21.825&21.825&21.732&21.788\\
         WikiLingua & 22.858&22.858&22.778&22.848\\
    \bottomrule
    \end{tabular}
    }
    \label{tab:single_rte_flan_t5}
\end{table*}





% \begin{table}[!htbp]
%     \centering
%     \caption{Results of model trained on RTE dataset. For RTE, CB and WiC, we report the results from development set. For other datasets, we report the results on test set. We list the accuracy on fine-tuning target task (RTE) on the first row. Here 1-shot Two-stage denotes running our two-stage fine-tune strategy on RTE dataset with 1-shot prompt. Note that the in-context performance of the prompt tuning case is the same as the pretrained model.}
%     \adjustbox{max width=\textwidth}{
%     \begin{tabular}{c|c|c|c|c|c|c|c|c}
%     \toprule
%          Datasets & \multicolumn{2}{c|}{Prompt-tuning} & \multicolumn{2}{c|}{Model Fine-tuning} & \multicolumn{2}{c|}{Two-stage (Ours)} &\multicolumn{2}{c}{1-shot Two-stage (Ours)}\\
%     \midrule
%          RTE & \multicolumn{2}{c|}{91.34} & \multicolumn{2}{c|}{92.06} & \multicolumn{2}{c|}{92.78}&\multicolumn{2}{c}{93.86}\\
%     \midrule
%          & 1-shot & 4-shots & 1-shot & 4-shots & 1-shot & 4-shots & 1-shot & 4-shots\\
%     \midrule
%          CB& 46.43 & 51.79 & 75.00 & 76.79 & 66.07 & 67.86&83.929&82.143\\
%          WiC & 49.687 & 49.687 & 50.627 & 50.157 & 51.411 & 53.605&51.254&50.627\\
%          triviaQA  & 17.582 & 19.022 & 0.018 & 0.018 & 17.643 & 18.66&17.82&19.623\\
%          web\_questions & 9.695 & 13.041 & 0& 0 & 11.073 & 13.189&10.138&12.106\\
%          WMT16\_ende & 3.974 & 8.83 & 0 & 0 & 2.018 & 3.694&2.256&4.894\\
%          WMT16\_enro & 1.818 & 3.918 & 0 & 0 & 0.704 & 0.959&0.87&1.868\\
%          XSum & 6.410 & 2.353 & 0 & 0 & 7.020 & 7.006&6.941&3.935\\
%          WikiLingua & 4.585 & 1.329 & 0 & 0 & 4.841 & 4.903&4.874&3.434\\
%     \bottomrule
%     \end{tabular}
%     }
%     \label{tab:single_rte}
% \end{table}

% \begin{table}[!htbp]
%     \centering
%     \caption{Results of model trained on WMT14 En-Fr dataset. For RTE, CB and WiC, we report the results from development set. For other datasets, we report the results on test set. We list the accuracy on fine-tuning target task (En-Fr) on the first row. Here 1-shot Two-stage denotes running our two-stage fine-tune strategy on En-Fr dataset with 1-shot prompt.}
%     \adjustbox{max width=\textwidth}{
%     \begin{tabular}{c|c|c|c|c|c|c|c|c}
%     \toprule
%          Datasets & \multicolumn{2}{c|}{Prompt-tuning} & \multicolumn{2}{c|}{Model Fine-tuning} & \multicolumn{2}{c|}{Two-stage (Ours)} & \multicolumn{2}{c}{1-shot Two-stage (Ours)}\\
%     \midrule
%          WMT14 En-Fr & \multicolumn{2}{c|}{39.28} & \multicolumn{2}{c|}{43.62} & \multicolumn{2}{c|}{41.3} & \multicolumn{2}{c}{41.19}\\
%     \midrule
%          & 1-shot & 4-shots & 1-shot & 4-shots & 1-shot & 4-shots & 1-shot & 4-shots\\
%     \midrule
%          CB& 46.43 & 51.79 & 25.6 & 23.214 & 41.071 & 57.143 & 41.071&53.571\\
%          WiC & 49.687 & 49.687 & 18.714 & 46.395 & 50.157 & 50.313&49.843&50.627\\
%          triviaQA  & 17.582 & 19.022 & 0.027 & 0.00 & 13.63 & 15.204&16.927&18.191\\
%          web\_questions & 9.695 & 13.041 & 0.049& 0.00 & 9.4 & 7.923&10.138&12.008\\
%          WMT16\_ende & 3.974 & 8.83 & 0.668 & 0.126 & 15.517 & 15.548&16.139&15.626\\
%          WMT16\_enro & 1.818 & 3.918 & 0.912 & 0.137 & 18.544 & 17.799&17.568&16.808\\
%          XSum & 6.410 & 2.353 & 0.181 & 0.063 & 1.493 & 0.65&3.407&4.362\\
%          WikiLingua & 4.585 & 1.329 & 0.034 & 0.005 & 1.142 & 0.524&4.215&4.727\\
%     \bottomrule
%     \end{tabular}
%     }
%     \label{tab:single_enfr}
% \end{table}

==> main_table_En-Fr_no_bold.tex <==
\begin{table}[!htbp]
    \centering
    \caption{In-context performance of model finetuned on WMT14 En-Fr. BLEU on the fine-tuned task is in the first row. The in-context performance of the pretrained model is the same as prompt-tuning. 
    % \michal{One of the two large tables could be moved to Appendix.}
    }
    \adjustbox{max width=\textwidth}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c}
    \toprule
         Datasets & \multicolumn{2}{c|}{Prompt-tuning} & \multicolumn{2}{c|}{Standard Fine-tuning} & \multicolumn{2}{c|}{ProMoT (Ours)} & \multicolumn{2}{c}{ProMoT + 1-shot (Ours)}\\
    \midrule
         WMT14 En-Fr & \multicolumn{2}{c|}{39.28} & \multicolumn{2}{c|}{41.796} & \multicolumn{2}{c|}{41.3} & \multicolumn{2}{c}{41.19}\\
    \midrule
         & 1-shot & 4-shots & 1-shot & 4-shots & 1-shot & 4-shots & 1-shot & 4-shots\\
    \midrule
         CB& 46.43 & 51.79 & 16.071 & 32.143 & 41.071 & 57.143 & 41.071&53.571\\
         WiC & 49.687 & 49.687 & 50.627 & 49.06 & 50.157 & 50.313&49.843&50.627\\
         triviaQA  & 17.582 & 19.022 & 3.2 & 3.147& 13.63 & 15.204&16.927&18.191\\
         web\_questions & 9.695 & 13.041 &0.886& 6.152 & 9.4 & 7.923&10.138&12.008\\
         WMT16\_ende & 3.974 & 8.83 & 0.808 & 0.175 & 15.517 & 15.548&16.139&15.626\\
         WMT16\_enro & 1.818 & 3.918 & 1.526 & 0.424 & 18.544 & 17.799&17.568&16.808\\
         XSum & 6.410 & 2.353 & 0.045 & 1.857 & 1.493 & 0.65&3.407&4.362\\
         WikiLingua & 4.585 & 1.329 & 0.03 & 0.429 & 1.142 & 0.524&4.215&4.727\\
    \bottomrule
    \end{tabular}
    }
    \label{tab:single_enfr}
\end{table}

==> main_table_RTE_no_bold.tex <==
\begin{table}[!htbp]
    \centering
    \caption{In-context performance of model finetuned on RTE. The accuracy on fine-tuned task (RTE) is in the first row. The in-context performance of the pretrained model is the same as prompt-tuning. 
    % \daliangli{are we still going to seperate pretraining with prompt-tuning?}
    }
    
    \adjustbox{max width=\textwidth}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c}
    \toprule
         Datasets & \multicolumn{2}{c|}{Prompt-tuning} & \multicolumn{2}{c|}{Standard Fine-tuning} & \multicolumn{2}{c|}{ProMoT (Ours)} &\multicolumn{2}{c}{ProMoT + 1-shot (Ours)}\\
    \midrule
         RTE & \multicolumn{2}{c|}{91.34} & \multicolumn{2}{c|}{92.06} & \multicolumn{2}{c|}{92.78}&\multicolumn{2}{c}{93.86}\\
    \midrule
         & 1-shot & 4-shots & 1-shot & 4-shots & 1-shot & 4-shots & 1-shot & 4-shots\\
    \midrule
         CB& 46.43 & 51.79 & 73.214 & 82.143 & 66.07 & 67.86&83.929&82.143\\
         WiC & 49.687 & 49.687 &50 & 50.157 & 51.411 & 53.605&51.254&50.627\\
         triviaQA  & 17.582 & 19.022 & 0.15 & 0.115 & 17.643 & 18.66&17.82&19.623\\
         web\_questions & 9.695 & 13.041 & 0.049& 0.049 & 11.073 & 13.189&10.138&12.106\\
         WMT16\_ende & 3.974 & 8.83 & 0 & 0 & 2.018 & 3.694&2.256&4.894\\
         WMT16\_enro & 1.818 & 3.918 & 0 & 0 & 0.704 & 0.959&0.87&1.868\\
         XSum & 6.410 & 2.353 & 0 & 0 & 7.020 & 7.006&6.941&3.935\\
         WikiLingua & 4.585 & 1.329 & 0 & 0 & 4.841 & 4.903&4.874&3.434\\
    \bottomrule
    \end{tabular}
    }
    \label{tab:single_rte}
\end{table}





% \begin{table}[!htbp]
%     \centering
%     \caption{Results of model trained on RTE dataset. For RTE, CB and WiC, we report the results from development set. For other datasets, we report the results on test set. We list the accuracy on fine-tuning target task (RTE) on the first row. Here 1-shot Two-stage denotes running our two-stage fine-tune strategy on RTE dataset with 1-shot prompt. Note that the in-context performance of the prompt tuning case is the same as the pretrained model.}
%     \adjustbox{max width=\textwidth}{
%     \begin{tabular}{c|c|c|c|c|c|c|c|c}
%     \toprule
%          Datasets & \multicolumn{2}{c|}{Prompt-tuning} & \multicolumn{2}{c|}{Model Fine-tuning} & \multicolumn{2}{c|}{Two-stage (Ours)} &\multicolumn{2}{c}{1-shot Two-stage (Ours)}\\
%     \midrule
%          RTE & \multicolumn{2}{c|}{91.34} & \multicolumn{2}{c|}{92.06} & \multicolumn{2}{c|}{92.78}&\multicolumn{2}{c}{93.86}\\
%     \midrule
%          & 1-shot & 4-shots & 1-shot & 4-shots & 1-shot & 4-shots & 1-shot & 4-shots\\
%     \midrule
%          CB& 46.43 & 51.79 & 75.00 & 76.79 & 66.07 & 67.86&83.929&82.143\\
%          WiC & 49.687 & 49.687 & 50.627 & 50.157 & 51.411 & 53.605&51.254&50.627\\
%          triviaQA  & 17.582 & 19.022 & 0.018 & 0.018 & 17.643 & 18.66&17.82&19.623\\
%          web\_questions & 9.695 & 13.041 & 0& 0 & 11.073 & 13.189&10.138&12.106\\
%          WMT16\_ende & 3.974 & 8.83 & 0 & 0 & 2.018 & 3.694&2.256&4.894\\
%          WMT16\_enro & 1.818 & 3.918 & 0 & 0 & 0.704 & 0.959&0.87&1.868\\
%          XSum & 6.410 & 2.353 & 0 & 0 & 7.020 & 7.006&6.941&3.935\\
%          WikiLingua & 4.585 & 1.329 & 0 & 0 & 4.841 & 4.903&4.874&3.434\\
%     \bottomrule
%     \end{tabular}
%     }
%     \label{tab:single_rte}
% \end{table}

% \begin{table}[!htbp]
%     \centering
%     \caption{Results of model trained on WMT14 En-Fr dataset. For RTE, CB and WiC, we report the results from development set. For other datasets, we report the results on test set. We list the accuracy on fine-tuning target task (En-Fr) on the first row. Here 1-shot Two-stage denotes running our two-stage fine-tune strategy on En-Fr dataset with 1-shot prompt.}
%     \adjustbox{max width=\textwidth}{
%     \begin{tabular}{c|c|c|c|c|c|c|c|c}
%     \toprule
%          Datasets & \multicolumn{2}{c|}{Prompt-tuning} & \multicolumn{2}{c|}{Model Fine-tuning} & \multicolumn{2}{c|}{Two-stage (Ours)} & \multicolumn{2}{c}{1-shot Two-stage (Ours)}\\
%     \midrule
%          WMT14 En-Fr & \multicolumn{2}{c|}{39.28} & \multicolumn{2}{c|}{43.62} & \multicolumn{2}{c|}{41.3} & \multicolumn{2}{c}{41.19}\\
%     \midrule
%          & 1-shot & 4-shots & 1-shot & 4-shots & 1-shot & 4-shots & 1-shot & 4-shots\\
%     \midrule
%          CB& 46.43 & 51.79 & 25.6 & 23.214 & 41.071 & 57.143 & 41.071&53.571\\
%          WiC & 49.687 & 49.687 & 18.714 & 46.395 & 50.157 & 50.313&49.843&50.627\\
%          triviaQA  & 17.582 & 19.022 & 0.027 & 0.00 & 13.63 & 15.204&16.927&18.191\\
%          web\_questions & 9.695 & 13.041 & 0.049& 0.00 & 9.4 & 7.923&10.138&12.008\\
%          WMT16\_ende & 3.974 & 8.83 & 0.668 & 0.126 & 15.517 & 15.548&16.139&15.626\\
%          WMT16\_enro & 1.818 & 3.918 & 0.912 & 0.137 & 18.544 & 17.799&17.568&16.808\\
%          XSum & 6.410 & 2.353 & 0.181 & 0.063 & 1.493 & 0.65&3.407&4.362\\
%          WikiLingua & 4.585 & 1.329 & 0.034 & 0.005 & 1.142 & 0.524&4.215&4.727\\
%     \bottomrule
%     \end{tabular}
%     }
%     \label{tab:single_enfr}
% \end{table}

==> seq_table.tex <==
\begin{table*}[ht]
    \centering
    \caption{Results for sequentially training first on RTE and then on En-Fr with ProMoT + 1-shot.
    % \daliangli{should we add the pretrained number here?}
    }
    \adjustbox{max width=0.8\linewidth}{
    \begin{tabular}{c|cc|c|c|c|c|c|c}
    \toprule
         Datasets & \multicolumn{2}{c|}{Pretrained Model} & \multicolumn{2}{c|}{ProMoT} & \multicolumn{2}{c|}{ProMoT} & \multicolumn{2}{c}{ProMoT + 1-shot}\\
         & \multicolumn{2}{c|}{}&\multicolumn{2}{c|}{+ 1-shot RTE} & \multicolumn{2}{c|}{+ 1-shot En-Fr} & \multicolumn{2}{c}{En-Fr after RTE} \\
    \midrule
         WMT14 En-Fr & \multicolumn{2}{c|}{1.98} & \multicolumn{2}{c|}{0.92} & \multicolumn{2}{c|}{41.19} & \multicolumn{2}{c}{41.33}\\
         RTE & \multicolumn{2}{c|}{47.65} & \multicolumn{2}{c|}{93.86} & \multicolumn{2}{c|}{53.43} & \multicolumn{2}{c}{90.98}\\
    \midrule
         & 1-shot & 4-shots &1-shot & 4-shots & 1-shot & 4-shots & 1-shot & 4-shots\\
    \midrule
         CB& 46.43 & 51.79 &83.93&82.14&41.07&53.57&82.14&80.36\\
         WiC & 49.69 & 49.69 &51.25 & 50.63 & 49.84&50.63&51.10&57.37\\
         triviaQA  & 17.58 & 19.02 &17.82 & 19.62 & 16.93 & 18.19 & 14.08 & 16.98\\
         web\_questions & 9.70 & 13.04 &10.14 & 12.11 & 10.14 & 12.01 & 9.40 & 11.71\\
         WMT16\_ende &  3.97 & 8.83 &2.26 & 4.89 & 16.14 & 15.63 & 18.13 & 17.90 \\
         WMT16\_enro & 1.82 & 3.92 &0.87 & 1.87 & 17.57 & 16.81 & 20.64 & 21.51\\
         XSum & 6.41 & 2.35 &6.94 & 3.94 & 3.41 & 4.36 & 3.19 & 3.96\\
         WikiLingua/en & 4.59 & 1.33 & 4.87 & 3.43 & 4.22 & 4.73&3.42&3.14\\
    \bottomrule
    \end{tabular}
    }
    \label{tab:seq_training}
\end{table*}
